ISO-RAG: Isoperimetric Noise Control for Retrieval-Augmented Generation

Retrieval-Augmented Generation (RAG) mitigates large language models (LLMs) hallucinations, yet conventional dense retrieval struggles with the complex reasoning paths of multi-hop question answering (QA). Graph-based RAG captures multi-step relationships but suffers from severe semantic drift and high online latency due to noisy global graph traversals. Thus, we propose ISO-RAG (ISOperimetric Retrieval-Augmented Generation), a geometry-aware RAG framework. By projecting the underlying knowledge graph into a hyperbolic Poincare ball to precompute node-wise isoperimetric profiles, ISO-RAG prunes spurious edges during retrieval, restricting the search space to a strictly localized subgraph. This topological purification regulates Personalized PageRank (PPR) diffusion driving the retrieval process, ensuring exact and low-latency convergence. Experiments on multi-hop QA benchmarks demonstrate that ISO-RAG outperforms state-of-the-art baselines by average absolute gains of 10.0% in retrieval recall and 4.3% in downstream exact match, achieving a superior accuracy-efficiency trade-off by fundamentally eliminating the latency bottleneck of global traversals. Our source code is available at https://github.com/ZaiizaiZHANG/ISO-RAG.

==> tables/casestudy.tex <==
\begin{table*}[t] % 使用 table* 使表格横跨两栏
\centering
% \small % 如果跨栏后依然拥挤，可取消注释此行将字号合法降至 9pt
% \setlength{\tabcolsep}{1mm} % 如果跨栏后列间距过宽，可取消注释此行合法压缩间距

\begin{tabular}{l cccc cccc cccc}
\toprule
\multirow{2.5}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{HotpotQA}} & \multicolumn{4}{c}{\textbf{2WikiMultihopQA}} & \multicolumn{4}{c}{\textbf{MuSiQue}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
& R@5 & R@10 & P@5 & P@10 & R@5 & R@10 & P@5 & P@10 & R@5 & R@10 & P@5 & P@10 \\
\midrule

% --- Sparse & Dense Baselines ---
BM25               & 62.70 & 75.25 & 25.08 & 15.05 & 39.80 & 48.20 & 18.42 & 11.08 & 27.00 & 32.15 & 10.64 & 6.34 \\
Flat Dense         & 81.90 & 87.95 & 32.76 & 17.59 & 69.43 & 71.58 & 31.82 & 16.39 & 52.40 & 58.95 & 20.54 & 11.57 \\
MDR                & 78.80 & 88.15 & 31.52 & 17.63 & 61.65 & 68.55 & 27.70 & 15.53 & 51.70 & 59.45 & 20.34 & 11.70 \\
\midrule

% --- Graph-based Baselines ---
Vanilla PPR        & 81.75 & 94.40 & 32.70 & 18.88 & 69.05 & 78.95 & 31.80 & 18.96 & 70.10 & 77.30 & 27.12 & 14.98 \\
GraphRAG           & 85.25 & 96.20 & 34.10 & 19.24 & 69.43 & 71.58 & 31.82 & 16.39 & 52.40 & 58.95 & 20.54 & 11.57 \\
GraphRAG+PPR       & 71.45 & 94.20 & 28.58 & 18.84 & 51.13 & 70.48 & 24.38 & 16.81 & 49.50 & 65.50 & 19.16 & 12.74 \\
LightRAG           & 87.30 & 97.20 & 34.92 & 19.44 & 77.93 & 88.80 & 35.92 & 20.95 & 55.05 & 67.05 & 21.60 & 13.16 \\
HippoRAG2          & 86.65 & 97.85 & 34.66 & 19.57 & 70.18 & 82.80 & 32.30 & 19.88 & 63.85 & 75.40 & 26.14 & 14.64 \\
HyperbolicRAG      & 85.30 & 96.85 & 34.12 & 19.37 & 70.45 & 78.38 & 32.34 & 18.55 & 55.35 & 76.05 & 21.70 & 14.70 \\
\midrule

% --- Ours ---
\textbf{ISO-RAG}   & \textbf{88.05} & \textbf{98.05} & \textbf{35.22} & \textbf{19.61} & \textbf{88.10} & \textbf{97.15} & \textbf{40.10} & \textbf{22.90} & \textbf{74.75} & \textbf{84.00} & \textbf{28.98} & \textbf{16.31} \\

\bottomrule
\end{tabular}
% AAAI 规定表格标题必须在表格主体下方
\caption{Retrieval performance comparison of Recall (R@) and Precision (P@) at top-5 and top-10 across three multi-hop datasets. Best results are \textbf{bolded}.}
\label{tab:retrieval_main}
\end{table*}

==> tables/casestudy2.tex <==
\begin{table}[t]
\centering
\caption{Qualitative Case Study from 2WikiMultihopQA. Query 2 illustrates a reasoning failure case: although ISO-PPR successfully retrieves the critical logical links, the LLM fails to deduce the correct final answer. Critical passages are marked with \checkmark, and irrelevant drift passages with $\times$.}
\label{tab:case_study2}
\small
\renewcommand{\arraystretch}{1.2}

% 摒弃宽大的设定，采用紧凑的列宽：1.5cm + 8cm + 3cm = 12.5cm
\begin{tabular}{@{} p{1.5cm} p{8cm} p{3cm} @{}}
\toprule

% 合并单元格的宽度必须和下面三列总和（12.5cm）严格保持一致！
\multicolumn{3}{@{} p{12.5cm} @{}}{\raggedright \textbf{Query 2 (Reasoning Failure Case):} \textit{"Do director of film Chicago 10 (Film) and director of film Black Oxen share the same nationality?"}} \\
\multicolumn{3}{@{} l @{}}{\textbf{Ground Truth Answer:} yes} \\
\midrule
\textbf{Method} & \textbf{Top-5 Retrieved Passages (Truncated Titles)} & \textbf{Qwen-Plus Answer} \\
\midrule
\multirow{5}{*}{\textbf{ISO-PPR}}
& [\checkmark] Chicago 10 (film) & \multirow{5}{*}{no} \\
& [\checkmark] Black Oxen & \\
& [\checkmark] \textbf{Brett Morgen} \textit{(Director of Chicago 10)} & \\
& [\checkmark] \textbf{Frank Lloyd} \textit{(Director of Black Oxen)} & \\
& [$\times$] Director X & \\
\bottomrule
\end{tabular}
\end{table}

==> tables/graph.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{Topological statistics of the dataset-specific evidence graphs.} Metrics include total node count ($|\mathcal{V}|$), total edge count ($|\mathcal{E}|$), and the average undirected degree.}
\label{tab:graph_stats}
\begin{tabular}{lccc}
\toprule
Dataset & Nodes ($|\mathcal{V}|$) & Edges ($|\mathcal{E}|$) & Average Degree \\
\midrule
HotpotQA & 9,758  & 44,442  & 9.1 \\
2WikiMultihopQA    & 5,813  & 33,881  & 11.7 \\
MuSiQue  & 10,218 & 130,921 & 25.6 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/hyperparameters.tex <==
\begin{table}[b]
\vspace{-1cm}
\centering
\small
\caption{Default retrieval profiles for ISO-RAG across different benchmarks.}
\label{tab:retrieval_profiles}
\begin{tabular}{lccccccccc}
\toprule
Dataset & \#Seeds & $\alpha$ & $\lambda_{\mathrm{g}}$ & $\lambda_{\mathrm{d}}$ & Dense Cand. & Pool Size & Seed Nbr. & Temp. ($\tau$) & $\beta$ \\
\midrule
HotpotQA & 3 & 0.85 & 0.48 & 0.52 & 80  & 120 & 18 & 8.0  & 0.35 \\
MuSiQue  & 3 & 0.85 & 0.90 & 0.10 & 150 & 240 & 32 & 25.0 & 0.10 \\
2Wiki    & 4 & 0.85 & 0.52 & 0.48 & 100 & 150 & 20 & 6.5  & 0.30 \\
\bottomrule

\end{tabular}
\end{table}

==> tables/retrieval_r.tex <==
\begin{table*}[t]
\centering
\caption{Retrieval Performance Comparison. We report Recall@5 (R@5) and Recall@10 (R@10) across three multi-hop datasets. The results demonstrate the superiority of \textbf{ISO-PPR} over traditional dense retrievers and recent GraphRAG baselines, particularly in deeper retrieval windows (R@10). The best results among practical retrieval methods are highlighted in \textbf{bold}.}
% 修复了这里的 label，改为 tab:retrieval_recall，与正文呼应
\label{tab:retrieval_recall} 
\small
\begin{tabular}{l cccccc}
\toprule
\multirow{2.5}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{HotpotQA}} & \multicolumn{2}{c}{\textbf{2WikiMultihop}} & \multicolumn{2}{c}{\textbf{MuSiQue}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& R@5 & R@10 & R@5 & R@10 & R@5 & R@10 \\
\midrule

% --- Sparse & Dense Baselines ---
BM25               & 62.70 & 75.25 & 39.80 & 48.20 & 27.00 & 32.15 \\
Flat Dense         & 81.90 & 87.95 & 69.43 & 71.58 & 52.40 & 58.95 \\
MDR                & 78.80 & 88.15 & 61.65 & 68.55 & 51.70 & 59.45 \\
\midrule

% --- Graph-based Baselines ---
Vanilla PPR        & 81.75 & 94.40 & 69.05 & 78.95 & 70.10 & 77.30 \\
GraphRAG           & 85.25 & 96.20 & 69.43 & 71.58 & 52.40 & 58.95\\
GraphRAG+PPR       & 71.45 & 94.20 & 51.13 & 70.48 & 49.50 & 65.50 \\
LightRAG           & 87.30 & 97.20 & 77.93 & 88.80 & 55.05 & 67.05 \\
HippoRAG2          & 86.65 & 97.85 & 70.18 & 82.80 & 63.85 & 75.40 \\
HyperbolicRAG & 85.30 & 96.85 & 70.45 & 78.38 & 55.35     & 76.05 \\
\midrule

% --- Ours ---
\textbf{ISO-PPR} & \textbf{88.05} & \textbf{98.05} & \textbf{88.10} & \textbf{97.15} & \textbf{74.75} & \textbf{84.00} \\

\bottomrule
\end{tabular}
\end{table*}


